DINER: Depth-aware Image-based NEural Radiance fields

We present Depth-aware Image-based NEural Radiance fields (DINER). Given a sparse set of RGB input views, we predict depth and feature maps to guide the reconstruction of a volumetric scene representation that allows us to render 3D objects under novel views. Specifically, we propose novel techniques to incorporate depth information into feature fusion and efficient scene sampling. In comparison to the previous state of the art, DINER achieves higher synthesis quality and can process input views with greater disparity. This allows us to capture scenes more completely without changing capturing hardware requirements and ultimately enables larger viewpoint changes during novel view synthesis. We evaluate our method by synthesizing novel views, both for human heads and for general objects, and observe significantly improved qualitative results and increased perceptual metrics compared to the previous state of the art. The code is publicly available for research purposes.

==> 5_results_old.tex <==
\begin{figure*}[ht!]
    \centering
    \def\svgwidth{0.95\linewidth}
    \input{figs/qual_eval_facescape_v2.pdf_tex}
    \caption{Qualitative comparison on FaceScape. IBRNet and KeypointNeRF produce artifacts for regions outside of the source images (\textcolor{mypink}{pink}). pixelNeRF handles these aspects better but produces blurry results. KeypointNeRF synthesizes heads with deformations (\textcolor{myorange}{orange}). Even without the perceptual loss, our method yields better results and adding the perceptual loss further emphasizes high-frequency details.
    }
    \label{fig:qual_comparison_facescape}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiments}
\label{sec:experiments}
%
\paragraph{Datasets}
The FaceScape dataset~\cite{yang2020facescape} contains more than 400k portrait photographs of 359 subjects under 20 different expressions captured with a rig of approximately 60 cameras. 
%
For each scan ground truth camera parameters and mesh reconstructions are provided which we use to render ground truth depth maps and foreground segmentations. 
%
Four of the captured subjects consented to the public display of their data which determined our training and validation splits.  
%
We apply post-processing in terms of color calibration and unification of depth ranges. 
%
% Unfortunately, FaceScape does not provide color-calibrated RGB images and since the dataset was capture on two different locations, the scene scales differ. 
% %
% We perform a post-capture color calibration by optimizing an image-wise affine color transformation to minimize the difference between the images and the vertex colors of the reconstructed meshes. Images for which this difference is too high are discarded. 
% %
% Further, we filter out images for which the rendered depth maps exceed \mbox{$[t_\text{near}, t_\text{far}] = [1.0m, 2.5m]$}.
%
We sample source view quadruples spanning horizontal and vertical angles of 45° and 30° respectively. Target views are sampled between the source views which results in $500k$ samples for training and $7k$ for validation. 
%
All images are cropped around the face region and rescaled to square crops of $256\times256$ px.
%\cite{wang2021ibrnet}
%\cite{yu2020pixelnerf}
%\cite{Mihajlovic:ECCV2022}

%
The DTU dataset~\cite{jensen2014large} is a large-scale multi-view data set of general scenes under controlled conditions. 
%
It contains 124 scenes with general objects captured from 49 to 64 positions including ground truth depth.
%
We follow the training/validation split convention proposed in \cite{yu2020pixelnerf}, adopt the preprocessing steps from \cite{ding2022transmvsnet}, and apply additional 2-fold downsampling to obtain images with resolution $256\times320$ px. 
%
Again, we sample source view quadruples spanning horizontal and vertical angles of $\approx 50°$ and $\approx 35°$ respectively which results in $30k$ samples for training and $5k$ for validation.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
\vspace{-0.35cm}
\paragraph{Baselines}
We compare our approach against the three state-of-the-art methods pixelNeRF~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet}, and KeypointNeRF~\cite{Mihajlovic:ECCV2022} for all of which the codebases are publicly available.
%
As pixelNeRF~\cite{yu2020pixelnerf} enables NeRFs to generalize across scenes by conditioning them on feature maps extracted from posed source views.
%
IBRNet~\cite{wang2021ibrnet} adds a transformer architecture and estimates blend weights for the source images instead of regressing color directly.
%
KeypointNeRF~\cite{Mihajlovic:ECCV2022} adds triangulated landmarks to guide the geometry estimation. Its dependence on keypoints makes the evaluation of KeypointNeRF on the DTU dataset impossible. 
%
In the official implementation, KeypointNeRF only renders the intersection of the source view frustums which we changed to their union in order to be able to cope with partial observations in source views. 
%
Since of-the-shelf keypoint detectors struggle with strong head rotations, we provide KeypointNeRF with ground truth keypoints.
%
We also evaluate a version of our method that does not include the bias-sensitive perceptual loss (see \Cref{sec:perc_loss}) which we train on 128 random rays per sample and a batch size of 16.
\vspace{-0.65cm}
\paragraph{Metrics}
We quantitatively evaluate the performance of our model through the pixel-wise Manhattan and Euclidean distances (L1) and (L2), structural similarity (SSIM), learned perceptual image patch similarity (LPIPS), and the peak signal-to-noise ratio (PSNR).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Results}
\paragraph{Novel View Synthesis}

\begin{table}
    \resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc} \toprule
\textbf{Method}& \textbf{LPIPS} $\downarrow$& \textbf{PSNR} $\uparrow$& \textbf{SSIM} $\uparrow$& \textbf{L1} $\downarrow$& \textbf{L2} $\downarrow$\\ \midrule
IBRNet \cite{wang2021ibrnet}& $0.159$& $22.7$& $0.89$& $0.025$& $0.006$\\
pixelNeRF \cite{yu2020pixelnerf}& $0.165$& $\color{dark-gray}\mathbf{23.54}$& $0.90$ & $0.021$& $\color{dark-gray}\mathbf{0.005}$\\
KeypointNeRF \cite{Mihajlovic:ECCV2022}& $0.148$& $18.39$& $0.86$& $0.036$& $0.017$\\\midrule
Ours w/o $\mathcal{L}_\text{perc}$& $\color{dark-gray}\mathbf{0.137}$& $\mathbf{24.40}$& $\mathbf{0.92}$ & $\mathbf{0.018}$& $\mathbf{0.004}$\\
Ours& $\mathbf{0.099}$& $22.42$& $\color{dark-gray}\mathbf{0.91}$ & $\color{dark-gray}\mathbf{0.020}$& $0.007$\\\bottomrule
\end{tabular}
}
\caption{Quantitative comparison on FaceScape.}
\label{tab:quant_comparison_facescape}
\end{table}

\Cref{fig:qual_comparison_facescape} displays a qualitative comparison between our method and the baselines on the FaceScape dataset~\cite{yang2020facescape}.
%
IBRNet~\cite{wang2021ibrnet} generally performs well in regions that project to a big surface on the source images, e.g., wrinkles in the mouth region for extreme expressions are synthesized convincingly. However, especially the eye regions project onto small areas and IBRNet fails to produce plausible results. Regions that lie outside of the source views show significant artifacts. 
%
pixelNeRF~\cite{yu2020pixelnerf} solves these cases better but tends to produce blurry results. 
%
KeypointNeRF~\cite{Mihajlovic:ECCV2022} synthesizes high-frequency details very plausibly but shows artifacts for regions outside of the source views and we also noticed severe deformations of the overall head shape (e.g. \Cref{fig:qual_comparison_facescape}, row 1 and 3). 
%
We attribute these deformations to the sparsity of guidance provided by triangulated landmarks. 
%
The dense guidance by depth maps in our method effectively solves this artifact and similarly to pixelNeRF, regressing color values directly allows us to plausibly synthesize regions that lie outside of the source views. At the same time, even without a perceptual loss, our method synthesizes high-frequency details better than IBRNet and pixelNeRF. Adding a perceptual loss emphasizes high-frequency detail synthesis even more and yields results that qualitatively outperform all baselines even though pixel-wise scores slightly worsen (see \Cref{tab:quant_comparison_facescape}). 
%
% We observe that our method outperforms all baselines on all metrics. Interestingly, we found that including the perceptual loss causes the L2 and PSNR scores to decline below pixelNeRF, even though the qualitative comparison shows significant improvements. We assign this observation to the well-known low-frequency-favouring property of these metrics.
%

%
Since depth maps can be estimated for arbitrary scenes, we can evaluate our model on general objects in the DTU dataset. The comparison in \Cref{fig:qual_comparison_dtu} demonstrates that our method outperforms all baselines by a significant margin. 
%
% While being primarily developed for image-based head synthesis, our method is not constrained to this domain since depth maps can be estimated for arbitrary images. This is a crucial property as it allows to synthesize additional objects that humans may interact with, e.g., a coffee mug in video-conferences. 
% %
% To showcase the universality of our approach, we also evaluate it on the general scenes of the DTU dataset. The qualitative comparison in \Cref{fig:qual_comparison_dtu} demonstrates that our method outperforms all baselines by a significant margin. Please note that KeypointNeRF cannot be used to render general scenes due to the lack of keypoints. We observed that the benefits of depth awareness are even more pronounced in the universal domain. 
% %
% For heads, even without depth-awareness the baseline models were able to learn a geometry prior with an impressive quality. For general scenes, this is not possible any longer and the effects of adding depth awareness increase even more. On the other side, we found that the benefits of adding a perceptual loss is more subtle even though the quantitative comparison in \Cref{tab:quant_comparison_dtu} reports a notably improved LPIPs score. 

\paragraph{Ablation Study}
\begin{figure*}[t]
    \centering
    \def\svgwidth{\linewidth}
    \input{figs/ablation.pdf_tex}
    \caption{Qualitative ablation study. Starting with pixelNeRF~\cite{yu2020pixelnerf} (first row, first column) as a baseline, we progressively add the components of our method and demonstrate their effects until we reach our final model (second row, last column). \todo{zoom in more to eye, heatmap}}
    \label{fig:ablation}
\end{figure*}

In this section, starting from pixelNeRF~\cite{yu2020pixelnerf} we progressively add our novel components and discuss their effects on the model performance. 
%
\Cref{fig:ablation} visualizes the qualitative effects by progressively introducing one new component per column. \Cref{tab:ablation} provides the quantitative evaluation. 
%
As the first step, we add depth awareness to pixelNeRF (\Cref{sec:depth_awareness}) which improves the overall synthesis quality and all scores. 
%
Introducing the perceptual loss $\mathcal{L}_\text{vgg}$ adds more high-frequency details but pixel-wise scores degrade.
%https://www.overleaf.com/project/62fdf7f88ace5acb60a36f66
% Please note that for evaluating $\mathcal{L}_\text{vgg}$ it is necessary to render patches of 64x64 px. This increases the number of MLP evaluations drastically which is why the batch size has to be reduced to 1 in order to fit the model on a GPU with 80 GB of memory. While adding $\mathcal{L}_\text{vgg}$ improves the LPIPS score, all pixel-wise metrics deteriorate, color shifts occur, and we observe smearing artifacts (third column in \Cref{fig:ablation}). 
%
Source feature extrapolation (\Cref{sec:feature_extrapolation}) counters smearing artifacts that occur in regions that are invisible in the source views. 
%
Color shifts that appeared after adding $\mathcal{L}_\text{vgg}$ can be eliminated with the anti-bias loss $\mathcal{L}_\text{ab}$ (\Cref{sec:perc_loss}). 
%
Depth-guided sampling (\Cref{sec:depth_guided_sampling}) increases the sampling density around the head surface and especially improves the synthesis quality around thin surfaces like ears. 
%
As a side effect, it also allows us to reduce the number of samples per ray and increase the batch size from 1 to 4 without changing GPU memory requirements. This slightly improves the qualitative results and consistently improves the scores of all metrics. 
%
%Note that similar effects could be achieved by training on 4 GPUs in parallel while requiring each GPU to be equipped with at least 70 GB of memory. 

\begin{table}
    \resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc} \toprule
\textbf{Method}& \textbf{L1} $\downarrow$& \textbf{L2} $\downarrow$& \textbf{LPIPS} $\downarrow$& \textbf{PSNR} $\uparrow$& \textbf{SSIM} $\uparrow$\\ \midrule
pixelNeRF \cite{yu2020pixelnerf} & $0.021$& $\mathbf{0.005}$& $0.16$& $23.54$& $0.90$\\
+ Depth Awareness & $\mathbf{0.020}$ & $\mathbf{0.005}$ & $0.15$ & $\mathbf{23.71}$ & $\mathbf{0.91}$ \\
+ Perc. Loss & $0.032$ & $0.008$ & $0.11$ & $21.66$ & $0.89$ \\
+ Source Feature Extrapolation  & $0.029$ & $0.008$ & $0.11$ & $21.96$ & $0.90$ \\
+ Bias-Sensitive Perc. Loss  & $0.022$ & $0.008$ & $0.11$ & $22.02$ & $0.90$ \\
+ Depth-Guided Sampling  & $0.023$ & $0.008$ & $0.12$ & $21.95$ & $0.90$ \\
+ Increased Batch Size (Ours) & $\mathbf{0.020}$ & $0.007$ & $\mathbf{0.10}$ & $22.42$ & $\mathbf{0.91}$  \\
\bottomrule
\end{tabular}
}
\caption{Quantitative Ablation Study on FaceScape.}
\label{tab:ablation}
\end{table}




\begin{figure*}[t]
    \centering
    \def\svgwidth{.9\linewidth}
    \input{figs/qual_eval_dtu.pdf_tex}
    \caption{Qualitative comparison on DTU.}
    \label{fig:qual_comparison_dtu}
\end{figure*}
